RSB-Pose: Robust Short-Baseline Binocular 3D Human Pose Estimation with Occlusion Handling

In the domain of 3D Human Pose Estimation, which finds widespread daily applications, the requirement for convenient acquisition equipment continues to grow. To satisfy this demand, we set our sights on a short-baseline binocular setting that offers both portability and a geometric measurement property that radically mitigates depth ambiguity. However, as the binocular baseline shortens, two serious challenges emerge: first, the robustness of 3D reconstruction against 2D errors deteriorates; and second, occlusion reoccurs due to the limited visual differences between two views. To address the first challenge, we propose the Stereo Co-Keypoints Estimation module to improve the view consistency of 2D keypoints and enhance the 3D robustness. In this module, the disparity is utilized to represent the correspondence of binocular 2D points and the Stereo Volume Feature is introduced to contain binocular features across different disparities. Through the regression of SVF, two-view 2D keypoints are simultaneously estimated in a collaborative way which restricts their view consistency. Furthermore, to deal with occlusions, a Pre-trained Pose Transformer module is introduced. Through this module, 3D poses are refined by perceiving pose coherence, a representation of joint correlations. This perception is injected by the Pose Transformer network and learned through a pre-training task that recovers iterative masked joints. Comprehensive experiments carried out on H36M and MHAD datasets, complemented by visualizations, validate the effectiveness of our approach in the short-baseline binocular 3D Human Pose Estimation and occlusion handling.

==> RSB-POSE/table/compare_with_sota_h36m.tex <==

\begin{table*}[t]
\caption{\textbf{Quantitative Comparison with SOTA methods on H36M datasets under MPJPE\_re and JDR metrics.} Scale is the input resolution of 2D backbone. The best results for each action within the same scale are highlighted in \textbf{bolded}.}
\label{tb:compare_with_sota_h36m_detail}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\begin{minipage}{\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|ccccccccccccccc|c}
\Xhline{0.12em}
\textbf{MPJPE\_re} (mm)  $\downarrow$ & 2D Backbone & Scale & Dir.           & Disc.          & Eat            & Greet          & Phone          & Photo          & Pose           & Purch.         & Sit            & SitD.          & Smoke          & Wait           & WalkD.         & Walk           & WalkT.         & Avg.           \\ \hline
TPPT \cite{ma_ppt_2022}                    & HRNet-W32   & 256   &38.27          & 42.88          & 34.94          & 35.83          & 44.62          & \textbf{33.91} & 41.13          & 48.31          & 56.19          & \textbf{45.79} & 48.95          & 37.75          & 36.45          & 43.71          & 35.71          & 42.10          \\
Epipolar -T. \cite{he_epipolar_2020}        & ResNet-50   & 256   & 36.79          & 39.14          & 34.69          & 34.34          & 39.58          & 39.77          & 32.70          & 35.34          & 41.41          & 47.24          & 39.42          & 37.12          & \textbf{34.55} & 38.61          & 33.05          & 37.97       \\
\rowcolor{colorSnd} RSB-Pose-ResNet50            & ResNet-50   & 256   & \textbf{24.90} & \textbf{31.18} & \textbf{26.64} & \textbf{27.22} & \textbf{33.95} & 35.10          & \textbf{25.97} & \textbf{31.72} & \textbf{37.37} & 56.51          & \textbf{35.43} & \textbf{31.10} & 36.79          & \textbf{27.41} & \textbf{27.03} & \textbf{32.80}\\ \hline
AdaFuse \cite{zhang_adafuse_2021}               & ResNet-152  & 384   & 24.93          & \textbf{27.30} & 26.48          & 26.53          & 29.53          & \textbf{21.92} & 25.54          & 30.39          & 45.93          & \textbf{30.98} & 28.64          & 27.29          & \textbf{23.18} & 28.82          & \textbf{23.24} & 28.52          \\
Algebraic-T. \cite{iskakov2019learnable}           & ResNet-152  & 384   & 26.83          & 31.89          & 24.14          & 27.76          & 28.88          & 26.78          & 25.54          & 29.93          & 31.33          & 42.46          & 29.56          & 28.31          & 32.84          & 26.18          & 26.59          & 29.44          \\
Volume-T. \cite{iskakov2019learnable}             & ResNet-152  & 384   & 27.26          & 31.95          & 26.76          & 30.35          & 31.57          & 32.74          & 26.64          & \textbf{28.45} & \textbf{30.76} & 41.18          & 32.28          & 27.82          & 33.62          & 30.28          & 30.52          & 30.97          \\

\rowcolor{colorFst} RSB-Pose-ResNet152           & ResNet-152  & 384   & \textbf{23.57} & 29.20          & \textbf{23.99} & \textbf{24.81} & \textbf{26.52} & 25.93          & \textbf{23.29} & 33.08          & 32.25          & 42.43          & \textbf{28.07} & \textbf{26.35} & 31.37          & \textbf{23.52} & 23.54          & \textbf{27.89} \\\Xhline{0.12em}
\end{tabular}}
\end{minipage}

\vspace{2em}

\begin{minipage}{\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccccccccccccccc|c}
 \Xhline{0.12em}
\textbf{JDR} (\%)  $\uparrow$& LShlder        & LElbow         & LWrist         & LHip           & LKnee          & LAnkle         & RShlder        & RElbow         & RWrist         & RHip           & RKnee          & RAnkle         & Pelvi          & Belly          & Neck           & Nose           & Head           & Avg.           \\ \hline
TPPT \cite{ma_ppt_2022}            & 95.32 & 90.285 & 80.21 & 96.20 & 93.32 & 85.63 & 92.74 & 89.42 & 81.33 & 99.43 & 94.98 & 91.96 & 100.00 & 98.38 & 97.67 & 97.44 & 99.02 & 93.32     \\
Epipolar -T. \cite{he_epipolar_2020}      & 93.82 & 93.7   & 91.70 & 99.15 & 96.99 & 93.34 & 94.05 & 93.16 & 91.36 & 99.34 & 97.24 & 95.57 & 100.00 & 99.95 & 99.31 & 99.47 & 99.50 & 96.40   \\
\rowcolor{colorSnd} RSB-Pose-ResNet50       & 94.64 & 94.31  & 92.55 & 92.48 & 95.30 & 95.37 & 92.98 & 95.09 & 94.84 & 95.32 & 95.32 & 93.49 & 96.01  & 96.01 & 95.76 & 96.08 & 96.42 & 94.82    \\ \hline
AdaFuse \cite{zhang_adafuse_2021}          & 95.79          & 93.91          & 89.12          & \textbf{96.41} & 93.67          & 92.40          & 94.20          & 93.03          & 89.08          & \textbf{96.48} & 94.13          & 93.04          & \textbf{96.65} & 95.40          & 95.94          & \textbf{96.54} & 96.38          & 94.25          \\
Algebraic-T. \cite{iskakov2019learnable}      & \textbf{96.47} & 94.91          & 93.58          & 95.21          & 95.87          & \textbf{95.78} & 94.59          & 95.51          & \textbf{96.45} & 96.26          & \textbf{96.31} & \textbf{96.38} & 96.26          & \textbf{96.38} & \textbf{96.40} & 96.42          & \textbf{96.61} & 95.81          \\
% Algebraic-T. \cite{iskakov2019learnable}      & \textbf{96.47} & 94.91          & 93.58          & 95.21          & 95.87          & \textbf{95.78} & 94.59          & 95.51          & \textbf{96.45} & 96.26          & \textbf{96.31} & \textbf{96.38} & 96.26          & \textbf{96.38} & \textbf{96.40} & 96.42          & \textbf{96.61} & 95.81          \\
\rowcolor{colorFst} RSB-Pose-ResNet152      & 96.19          & \textbf{96.06} & \textbf{94.93} & 94.13          & \textbf{96.24} & 95.30          & \textbf{95.78} & \textbf{96.26} & 96.38          & 96.29          & 96.18          & 95.60          & 96.19          & 96.08          & 96.24          & 96.42          & \textbf{96.61} & \textbf{95.93} \\ \Xhline{0.12em}
\end{tabular}}
\end{minipage}

\end{table*}

==> RSB-POSE/table/compare_with_sota_h36m_sim2d.tex <==
\begin{table*}[]
\caption{\textbf{Quantitative Comparison with SOTA methods on H36M datasets under SIM\_cos.} }
\label{tb:compare_with_sota_h36m_sim2d}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccccccccccccccc|c}
\Xhline{0.12em}
\textbf{SIM\_cos} $\uparrow$  & LShlder & LElbow & \nd LWrist & LHip & LKnee & LAnkle & RShlder & RElbow & \nd RWrist & RHip & RKnee & RAnkle & Pelvi & Belly & Neck & Nose & Head & \textbf{Avg.} \\ \hline
Algebraic-T. \cite{iskakov2019learnable}       & 0.89    & 0.73   & \nd0.67   & 0.75 & 0.88  & 0.96   & 0.79    & 0.80   & \nd0.62   & 0.75 & 0.86  & 0.83   & 0.69  & 0.86  & 0.75 & 0.80 & 0.78 & \textbf{0.79} \\
RSB-Pose-ResNet152 & 0.92    & 0.92   & \nd0.90   & 0.86 & 0.96  & 0.96   & 0.93    & 0.90   & \nd0.90   & 0.90 & 0.97  & 0.98   & 0.89  & 0.94  & 0.92 & 0.96 & 0.99 & \textbf{0.94}\\
\Xhline{0.12em}
\end{tabular}
}
\end{table*}

==> RSB-POSE/table/compare_with_sota_mhad.tex <==
\begin{table*}[b]
\caption{\textbf{Quantitative Comparison with SOTA methods on MHAD datasets under MPJPE\_ab and JDR metrics.} Scale is the input resolution of 2D backbone. The best results for each action within the same scale are highlighted in \textbf{bolded}.}
\label{tb:compare_with_sota_mhad_detail}
% \setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\begin{minipage}{\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|ccccccccccc|c}
\Xhline{0.12em}
\textbf{MPJPE\_ab} (mm) $\downarrow$& 2D Backbone & Scale & A01            & A02            & A03            & A04            & A05            & A06            & A07            & A08            & A09            & A10            & A11            & Avg.           \\ \hline
TPPT \cite{ma_ppt_2022}                     & HRNet-W32   & 256   & 149.90         & 457.33         & 156.21         & 232.54         & 168.72         & 149.11         & 146.27         & 487.09         & 169.24         & 215.90         & 266.16         & 209.03         \\
Epipolar -T.  \cite{he_epipolar_2020}          & ResNet-50   & 256   & 85.35          & 89.63          & 95.80          & 87.03          & 96.66          & 89.03          & 80.33          & 100.86         & 88.87          & 96.06          & 94.05          & 90.73          \\
\rowcolor{colorSnd} RSB-Pose-ResNet50             & ResNet-50   & 256   & \textbf{27.77} & \textbf{32.31} & \textbf{32.50} & \textbf{31.17} & \textbf{34.12} & \textbf{27.09} & \textbf{24.39} & \textbf{41.99} & \textbf{34.19} & \textbf{39.17} & \textbf{33.53} & \textbf{32.16} \\ \hline
AdaFuse        \cite{zhang_adafuse_2021}         & ResNet-152  & 384   & 194.07         & 203.27         & 154.87         & 169.93         & 197.33         & 197.57         & 170.74         & 243.68         & 206.98         & 197.38         & 200.32         &  189.16         \\
Algebraic-T. \cite{iskakov2019learnable}           & ResNet-152  & 384   & 40.61          & 71.38          & 55.74          & 43.39          & 53.36          & 35.97          & 43.79          & 91.83          & 50.32          & 52.99          & 46.40          & 51.69          \\
Volume-T.   \cite{iskakov2019learnable}            & ResNet-152  & 384   & 33.40          & 32.70          & 32.53          & 31.49          & 31.65          & 28.01          & \textbf{26.95} & 77.05          & 37.83          & 39.68          & 33.91          &  34.67          \\
\rowcolor{colorFst} RSB-Pose-ResNet152            & ResNet-152  & 384   & \textbf{27.11} & \textbf{28.58} & \textbf{28.74} & \textbf{29.47} & \textbf{28.53} & \textbf{25.22} & 38.28          & \textbf{30.61} & \textbf{35.60} & \textbf{31.67} & \textbf{31.67} & \textbf{29.33}
\\\Xhline{0.12em}
\end{tabular}}
\end{minipage}

\vspace{2em}

\begin{minipage}{\textwidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|ccccccccccc|c}
\Xhline{0.12em}
\textbf{JDR} (\%) $\uparrow$& 2D Backbone & Scale & Shlder         & Elbow          & Wrist          & Hip            & Knee           & Ankle          & Pelvi          & Belly          & Neck           & Nose           & Head           & Avg.           \\ \hline
TPPT  \cite{ma_ppt_2022}            & HRNet-W32   & 256   & 90.51          & 78.88          & 63.77          & 96.13          & 94.41          & 92.56          & 96.73          & 93.97          & 91.39          & 88.58          & 87.29          & 87.67          \\
Epipolar -T.  \cite{he_epipolar_2020}   & ResNet-50   & 256   & 93.24          & 86.49          & 75.72          & 98.09          & 98.27          & 96.44          & \textbf{98.03} & 93.91          & 90.22          & 90.13          & 91.02          & 91.75          \\
\rowcolor{colorSnd} RSB-Pose-ResNet50      & ResNet-50   & 256   & \textbf{97.12} & \textbf{97.50} & \textbf{95.78} & \textbf{99.95} & \textbf{99.96} & \textbf{99.98} & 58.85          & \textbf{99.64} & \textbf{99.80} & \textbf{99.89} & \textbf{99.30} & \textbf{96.35} \\ \hline
AdaFuse  \cite{zhang_adafuse_2021}        & ResNet-152  & 384   & 84.30          & 76.22          & 66.83          & 90.96          & 93.93          & 97.86          & 90.53          & 84.39          & 81.18          & 78.86          & 56.04          & 83.46          \\
Algebraic-T. \cite{iskakov2019learnable}    & ResNet-152  & 384   & 91.30          & 93.27          & 91.78          & 99.81          & 99.91          & 99.87          & \textbf{99.74} & 97.20          & 97.59          & 92.95          & 91.73          & 95.95          \\
\rowcolor{colorFst} \fs RSB-Pose-ResNet152     & ResNet-152  & 384   & \textbf{98.51} & \textbf{99.26} & \textbf{97.49} & \textbf{99.98} & \textbf{99.97} & \textbf{99.99} & 67.71          & \textbf{99.92} & \textbf{99.92} & \textbf{99.35} & \textbf{98.58} & \textbf{97.40}
\\ \Xhline{0.12em}
\end{tabular}}
\end{minipage}

\end{table*}

==> RSB-POSE/table/impact_of_each_module_1.tex <==
\begin{table}[]
\caption{\textbf{The Impact of Each Module.} ``notocc`` and ``occ`` denote the keypoints that are not occluded and occluded, respectively.}
\label{tb:impact_of_each_module}
\centering
\setlength{\tabcolsep}{1.4pt}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\Xhline{0.15em}
\multicolumn{1}{c|}{\multirow{2}{*}{method}} & \multicolumn{2}{c}{SCG}                                    & \multicolumn{1}{c|}{Pretrained} & \multicolumn{3}{c|}{MPJPE\_ab (mm)}                                                  & \multicolumn{3}{c}{MPJPE\_re (mm)}                                                  \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c}{w/o mask} & \multicolumn{1}{c}{w/ mask} & \multicolumn{1}{c|}{PT}         & \multicolumn{1}{c}{all} & \multicolumn{1}{c}{notocc} & \multicolumn{1}{c|}{occ} & \multicolumn{1}{c}{all} & \multicolumn{1}{c}{notocc} & \multicolumn{1}{c}{occ} \\\hline
Baseline-50                                 &                              &                             &                                & 63.18                   & 62.99                      & 73.13                   & 88.89                   & 88.71                      & 98.31                   \\ \hline
\multirow{3}{*}{PoseTRoB-50}                                  & \checkmark                            &                             &                                & 47.61                   & 47.42                      & 54.50                   & 59.09                   & 58.95                      & 64.24                   \\
                                            &                              & \checkmark                           &                                & 35.40                   & 35.25                      & 40.73                   & 39.78                   & 39.56                      & 47.70                   \\
                                            &                              & \checkmark                           & \checkmark                              & 32.10                   & 31.94                      & 37.78                   & 37.59                   & 37.36                      & 46.19                   \\ \hline
Baseline-152                                &                              &                             &                                & 59.00                   & 58.79                      & 69.99                   & 77.19                   & 77.01                      & 86.61                   \\ \hline
\multirow{3}{*}{PoseTRoB-152}  & \checkmark                            &                             &                                & 30.40                   & 30.24                      & 36.13                   & 35.82                   & 35.58                      & 44.27                   \\
                                            &                              & \checkmark                           &                                & 29.78                   & 29.60                      & 36.19                   & 34.81                   & 34.58                      & 43.42                   \\
                                            &                              & \checkmark                           & \checkmark                              &                         &                            &                         &                         &                            &         \\\Xhline{0.15em}               
\end{tabular}}
\end{table}

==> RSB-POSE/table/impact_of_mask_ratio.tex <==
\begin{table}[h]
\caption{\textbf{The Impact of Mask Ratio.} $Mask\_Ratio = 0$ refers to Baseline-50. PPT with different mask ratios are directly added to refine the initial 3D pose from baseline.}
\label{tb:impact_of_mask_ratio}
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cccccc}
\Xhline{0.12em}
Mask\_Ratio (Iter\_T=1)    & 0.0  & 0.1  & 0.2  & 0.3  & 0.4  & 0.5  \\ \hline
MPJPE\_ab (mm) $\downarrow$ & 63.18 & 65.87 & 67.63 & 65.23 & 63.80 & 66.15
\\
MPJPE\_re (mm) $\downarrow$ & 62.70 & 63.39 & 64.91 & 62.83 & 62.25 & 64.15
\\\Xhline{0.12em}
\end{tabular}}

\end{table}

==> RSB-POSE/table/validation_of_PT_occ.tex <==
\begin{table}[t]
\caption{\textbf{The impact of pretrained PT refinement in MHAD\_occ.} ``initial" and ``refined" refer to the 3D pose, with ``initial" indicating the original pose and "refined" indicating the pose that is optimized by the PPT.}
\label{tb:validation_of_pt_occ}
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc}
\Xhline{0.12em}
\multicolumn{1}{l|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c|}{MPJPE\_ab (mm) $\downarrow$}                             & \multicolumn{2}{c}{MPJPE\_re (mm) $\downarrow$}                             \\
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c}{initial} & \multicolumn{1}{c|}{refined} & \multicolumn{1}{c}{initial} & \multicolumn{1}{c}{refined} \\ \hline
TPPT \cite{ma_ppt_2022}                                      & 185.68                      & 164.08                      & 205.99                      & 170.75                      \\
Epipolar -T. \cite{he_epipolar_2020}                               & 92.30                       & 86.12                       & 93.02                       & 84.71                       \\
Adafuse \cite{zhang_adafuse_2021}                                    & 144.72                      & 125.08                      & 141.63                      & 120.08                      \\
Algebraic-T. \cite{iskakov2019learnable}                               & 66.30                       & 68.42                       & 61.73                       & 60.06                       \\
Volume-T. \cite{iskakov2019learnable}                                & 43.97                       & 43.18                       & 30.25                       & 30.22                      \\ \Xhline{0.12em}
\end{tabular}}
\end{table}
